Hadronic form factors for rare semileptonic $B$ decays

We discuss first results for the computation of short distance contributions to semileptonic form factors for the rare $B$ decays $B \to K^{*} \ell^+\ell^-$ and $B_s \to \phi \ell^+ \ell^-$. Our simulations are based on RBC/UKQCD's $N_f=2+1$ ensembles with domain wall light quarks and the Iwasaki gauge action. For the valence $b$-quark we chose the relativistic heavy quark action.

==> Proceedings_aux <==
\relax 
\global\@todotoctrue
\citation{Lee:1973iz,Donoghue:1978cj}
\citation{Grinstein:1987vj,Grinstein:1990tj,Buras:1993xp,Ciuchini:1993ks,Ciuchini:1993fk,Ciuchini:1994xa}
\citation{Buras:2002tp,Gambino:2003zm,Altmannshofer:2008dz}
\citation{Grinstein:2004vb,Beylich:2011aq}
\citation{Lyon:2014hpa}
\citation{Aaij:2015esa,LHCb:2015dla}
\citation{Descotes-Genon:2013wba,Altmannshofer:2013foa,Altmannshofer:2014rta}
\citation{Horgan:2013pva,Horgan:2013hoa,Horgan:2015vla}
\citation{Bouchard:2013mia}
\citation{Bailey:2015dka,Du:2015tda}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{2}}
\newlabel{eq:tf-2}{{1.2}{2}}
\newlabel{eq:tf-1}{{1.3}{2}}
\global\@todotoctrue
\citation{Allton:2008pn,Aoki:2010dy}
\citation{Shamir:1993zy,Furman:1994ky}
\citation{Christ:2006us}
\citation{Aoki:2012xaa}
\citation{Allton:2008pn,Aoki:2010dy}
\citation{Blum:2014tka}
\citation{Blum:2014tka}
\citation{Allton:2008pn,Aoki:2010dy}
\citation{Blum:2014tka}
\citation{Blum:2014tka}
\citation{Altmannshofer:2008dz}
\newlabel{tab:1}{{2}{3}}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Parameters of the calculation. We use the coarse ensembles generated by the RBC and UKQCD collaboration \cite  {Allton:2008pn, Aoki:2010dy} with 2+1 flavor domain-wall fermions and Iwasaki gauge actions. The domain-wall fermions are created with fifth dimension $L_s=16$ and domain-wall height $M_5=1.8$. Values for the inverse lattice spacing and the quark and meson masses are taken from the refined analysis \cite  {Blum:2014tka}; $am_l$ labels the mass of the light sea-quark, $am_h$ the mass of the heavy sea quark, and $am_s^\prime $ the mass of the near physical strange quark mass. The physical value of the strange quark mass is $am_s=0.03224(18)$ \cite  {Blum:2014tka}.}}{3}}
\@writefile{toc}{\contentsline {section}{\numberline {2}Computational setup}{3}}
\newlabel{Sec.Setup}{{2}{3}}
\newlabel{eq:1}{{2.1}{3}}
\newlabel{eq:2}{{2.4}{3}}
\citation{Aoki:2012xaa}
\global\@todotoctrue
\citation{Edwards:2004sx}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Three point correlator function used to obtain the $B\to V$ form factors. The single and double lines correspond to light and $b$-quark propagators, respectively.}}{4}}
\newlabel{fig:3pt}{{1}{4}}
\newlabel{eq:ratio}{{2.5}{4}}
\newlabel{eq.3pt}{{2.7}{4}}
\newlabel{eq:2pt-0}{{2.8}{4}}
\@writefile{toc}{\contentsline {section}{\numberline {3}First results}{4}}
\newlabel{Sec.Results}{{3}{4}}
\global\@todotoctrue
\citation{ElKhadra:2001rv}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Bare form factor $f_{A_1}$ for the $B_s\to \phi \ell ^+\ell ^-$ decay at zero momentum for four different source-sink separations $t_{sink}$ on the coarse $a\approx 0.11$fm ensemble with $am_l=0.005$.}}{5}}
\newlabel{fig:source-sink}{{2}{5}}
\@writefile{toc}{\contentsline {section}{\numberline {4}Summary and outlook}{5}}
\newlabel{Sec.Summary}{{4}{5}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Bare form factors $f_V,\ f_{A_0},\ f_{A_1},\ f_{A_2}$ for $B_s \to \phi \ell ^+\ell ^-$ decays. Left: plateau fits for the coarse ensemble with $am_l=0.005$, right: extracted form factor values vs.\nobreakspace  {}$q^2$ in GeV obtained on both coarse ensembles, $am_l = 0.005$ and $am_l = 0.010$.}}{6}}
\newlabel{fig:A1}{{3}{6}}
\bibdata{../B_meson}
\bibcite{Lee:1973iz}{{1}{}{{}}{{}}}
\bibcite{Donoghue:1978cj}{{2}{}{{}}{{}}}
\bibcite{Grinstein:1987vj}{{3}{}{{}}{{}}}
\bibcite{Grinstein:1990tj}{{4}{}{{}}{{}}}
\bibcite{Buras:1993xp}{{5}{}{{}}{{}}}
\bibcite{Ciuchini:1993ks}{{6}{}{{}}{{}}}
\bibcite{Ciuchini:1993fk}{{7}{}{{}}{{}}}
\bibcite{Ciuchini:1994xa}{{8}{}{{}}{{}}}
\bibcite{Buras:2002tp}{{9}{}{{}}{{}}}
\bibcite{Gambino:2003zm}{{10}{}{{}}{{}}}
\bibcite{Altmannshofer:2008dz}{{11}{}{{}}{{}}}
\bibcite{Grinstein:2004vb}{{12}{}{{}}{{}}}
\bibcite{Beylich:2011aq}{{13}{}{{}}{{}}}
\bibcite{Lyon:2014hpa}{{14}{}{{}}{{}}}
\bibcite{Aaij:2015esa}{{15}{}{{}}{{}}}
\bibcite{LHCb:2015dla}{{16}{}{{}}{{}}}
\bibcite{Descotes-Genon:2013wba}{{17}{}{{}}{{}}}
\bibcite{Altmannshofer:2013foa}{{18}{}{{}}{{}}}
\bibcite{Altmannshofer:2014rta}{{19}{}{{}}{{}}}
\bibcite{Horgan:2013pva}{{20}{}{{}}{{}}}
\bibcite{Horgan:2013hoa}{{21}{}{{}}{{}}}
\bibcite{Horgan:2015vla}{{22}{}{{}}{{}}}
\bibcite{Bouchard:2013mia}{{23}{}{{}}{{}}}
\bibcite{Bailey:2015dka}{{24}{}{{}}{{}}}
\bibcite{Du:2015tda}{{25}{}{{}}{{}}}
\bibcite{Allton:2008pn}{{26}{}{{}}{{}}}
\bibcite{Aoki:2010dy}{{27}{}{{}}{{}}}
\bibcite{Shamir:1993zy}{{28}{}{{}}{{}}}
\bibcite{Furman:1994ky}{{29}{}{{}}{{}}}
\bibcite{Christ:2006us}{{30}{}{{}}{{}}}
\bibcite{Aoki:2012xaa}{{31}{}{{}}{{}}}
\bibcite{Blum:2014tka}{{32}{}{{}}{{}}}
\bibcite{Edwards:2004sx}{{33}{}{{}}{{}}}
\bibcite{ElKhadra:2001rv}{{34}{}{{}}{{}}}
\bibstyle{apsrev4-1ow}
\providecommand\NAT@force@numbers{}\NAT@force@numbers
\@writefile{toc}{\contentsline {paragraph}{Acknowledgements}{7}}

